Cutting Quantum Circuits to Run on Quantum and Classical Platforms

Quantum computing (QC) offers a new computing paradigm that has the potential to provide significant speedups over classical computing. Each additional qubit doubles the size of the computational state space available to a quantum algorithm. Such exponentially expanding reach underlies QC's power, but at the same time puts demanding requirements on the quantum processing units (QPU) hardware. On the other hand, purely classical simulations of quantum circuits on either central processing unit (CPU) or graphics processing unit (GPU) scale poorly as they quickly become bottlenecked by runtime and memory. This paper introduces CutQC, a scalable hybrid computing approach that distributes a large quantum circuit onto quantum (QPU) and classical platforms (CPU or GPU) for co-processing. CutQC demonstrates evaluation of quantum circuits that are larger than the limit of QPU or classical simulation, and achieves much higher quantum circuit evaluation fidelity than the large NISQ devices achieve in real-system runs.

==> text/Acknowledgement.tex <==
\section*{ACKNOWLEDGMENT}

We thank A, B, and C. This work was supported in part by a grant from XYZ.

==> text/FD_Results.tex <==
\subsection{Full Definition Query}\label{sec:full_definition_results}
\setlength{\belowcaptionskip}{-5pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fd_runtime.pdf}
    \caption{CutQC executes benchmark circuits mapped to quantum devices with up to $\frac{3}{4}$ of the number of qubits in the input circuits.
    The horizontal axis shows the number of qubits in the input circuit.
    The vertical axis shows the postprocessing runtime of the full definition reconstruction.
    CutQC enables FD query almost always faster than classical simulations do.
    CutQC offers an average of 60X to 8600X runtime speedup over classical simulation alternatives for different benchmarks.
    GPU is the fastest backend as expected.}
    \label{fig:fd_expand}
\end{figure}

The size of quantum devices serves as the baseline to
demonstrate CutQC's ability to expand the size of quantum circuits.
The Qiskit runtime of classically simulating the benchmark circuits serves as the
baseline to demonstrate CutQC's ability to speed up quantum circuit evaluations.

The experiments in Figure~\ref{fig:fd_expand} show the effect of different benchmarks, quantum circuit sizes, and quantum computer sizes on postprocessing runtime.
We used 10-, 15-, 20-, and 25-qubit quantum computers and ran benchmark circuits larger than the devices in FD query using 16 compute nodes for postprocessing.
We achieve an average of 60X to 8600X runtime speedup over classical simulation for our benchmarks.

The type of benchmarks, quantum circuit sizes, and available quantum computer sizes are all important contributors to runtime.
First, some benchmarks are harder to cut and require more postprocessing overhead.
Specifically, \textit{Supremacy} \textit{AQFT} are more densely connected circuits and generally require more postprocessing.
Second, larger quantum circuits generally require more postprocessing.
The reason is that executing quantum circuits that significantly exceed the available quantum resources has to rely more on classical computing resources.
In some cases, the classical postprocessing incurred outweighs any benefit from having quantum computers,
and the resulting runtime is longer than classical simulation.
Third, having larger quantum computers generally improves the runtime.
However, having larger quantum computers faces diminishing returns.
The postprocessing overhead eventually plateaus when the quantum computer is large enough to support an efficient partitioning of the circuit.
For example, the 5*7 \textit{Supremacy} circuit is cut into 2 subcircuits with 5 cuts on both 20- and 25-qubit computers and has similar runtime.
